Skew Howe duality for Types $\mathbf{BD}$ via $q$-Clifford algebras

We extend a quantized skew Howe duality result for Type $\mathbf{A}$ algebras to orthogonal types via a seesaw. We develop an operator commutant version of the First Fundamental Theorem of invariant theory for $U_q(\mathfrak{so}_n)$ using a double centralizer property inside a quantized Clifford algebra. We obtain a multiplicity-free decomposition of tensor powers of the $U_q(\mathfrak{so}_{2n})$ spin representation by explicitly computing joint highest weights with respect to an action of $U_q(\mathfrak{so}_{2n}) \otimes U_q'(\mathfrak{so}_m)$. Clifford algebras are an essential feature of our work: they provide a unifying framework for classical and quantized skew Howe duality results that can be extended to include orthogonal algebras of types $\mathbf{BD}$.

==> source/alpha/notation_conventions.tex <==
%\documentclass[../../main.tex]{subfiles}
%\begin{document}

We will use $e_i$ throughout to denote the standard basis of $\mathbb{R}^n$.

In this section we fix our notation for Lie algebras and recall some definitions. \longer{Let $\lieg$ denote either the reductive complex Lie algebra $\mathfrak{gl}_n$, or a finite-dimensional complex semisimple Lie algebra. We will mainly consider the cases $\lieg = \mathfrak{gl}_n, \mathfrak{so}_n$, and $\mathfrak{sp}_n$.} 

\paragraph{Lie algebra presentation}
Following \cite{chari_pressley_1994}, we use the \textit{Chevalley presentation} throughout. If $\lieg$ is a complex semisimple Lie algebra, we let $A = [a_{ij}]$ denote its \textit{generalized Cartan matrix}.  We let $D = \mathrm{diag}(d_1, \ldots, d_r)$ denote the diagonal matrix of root lengths such that $DA$ is symmetric positive definite. Recall $a_{ii} = 2$ and $a_{ij} \leq 0$ whenever $i\neq j$.
	
The semisimple algebra $\lieg$ is generated by $H_i, E_i$, and $F_i$, for $i = 1, \ldots, r$, subject to the relations
\begin{equation}\label{chevalley presentation of g}
	\begin{gathered}
	[H_i, H_j] = 0, \quad [H_i, E_j] = a_{ij} E_j, \quad [H_i, F_j] = -a_{ij} F_j, \quad [E_i, F_j] = \delta_{ij} H_i,  \\
	\end{gathered}
\end{equation}
along with the \textit{Serre relations} for $i \neq j$:
\begin{equation}\label{Serre rels of g}
	(\mathrm{ad}_{E_i})^{1-a_{ij}}(E_j) = 0, \quad \text{and} \quad (\mathrm{ad}_{F_i})^{1-a_{ij}}(F_j) = 0
\end{equation}
\begin{remark}
	Authors like Jantzen \cite{J}, Lusztig \cite{lusztig_1988}, and Sawin \cite{sawin_1996} prefer the notation $X_i^+ = E_i$ and $X_i^- = F_i$, suggestive of positive and negative roots in general, and of ``raising'' and ``lowering'' operators in this context.
\end{remark}

We will denote by $\Ug$ the \textit{universal enveloping algebra} associated to $\lieg$\longer{ \cite[Chapter~10]{Bump}. This associative unital algebra has the same generators as $\lieg$, subject to relations in \eqref{chevalley presentation of g}, where in this case $[A, B] = AB - BA$ denotes the usual algebra commutator. The generators are also subject to the Serre relations \eqref{Serre rels of g}, which are written in this context as
\begin{equation*}\label{classical Serre relations}
	\sum_{k=0}^{1-a_{ij}}(-1)^k \binom{1-a_{ij}}{k} (X_i)^k X_j (X_i)^{1- a_{ij}-k} = 0.
\end{equation*}
In the last equality $X$ is either an $E$ or an $F$}.

Now fix the \textit{Cartan subalgebra} $\mathfrak{h}$ generated by the $H_i$\longer{ and let $\mathfrak{b}$ denote the \textit{Borel subalgebra} containing $\mathfrak{h}$}. The \textit{simple roots} of $\lieg$ are the linear functionals $\alpha_i\colon \mathfrak{h} \to \mathbb{C}$ satisfying
\begin{equation*}
	\alpha_i(H_j) = a_{ji}.
\end{equation*}
\longer{We use $\varPhi$ to denote the set of simple roots and we set 
\begin{equation*}
	\mathcal{Q} = \bigoplus_{\alpha \in \varPhi} \mathbb{Z} \alpha 
	\quad \text{and} \quad 
	\mathcal{Q}^+ = \bigoplus_{\alpha \in \varPhi} \mathbb{Z}_+ \alpha.
\end{equation*}}
We let
\begin{equation}\label{weights and dominant weights}
	\mathcal{P} = \{ \lambda \in \mathfrak{h}^* \mid \lambda(H_i) \in \mathbb{Z} \} \quad \text{and} \quad \mathcal{P}^+ = \{ \lambda \in \mathfrak{h}^* \mid \lambda(H_i) \in \mathbb{Z}_+ \}
\end{equation}
denote the lattice of \textit{weights} and \textit{dominant weights}, respectively.

\paragraph{Bilinear form}
When $\lieg$ is semisimple, there exists a unique non-degenerate symmetric invariant bilinear form $\langle , \rangle\colon \lieg \times \lieg \to \mathbb{C}$ such that
\begin{gather*}
\begin{split}
	\langle H_i, H_j \rangle = \inv{d_j} a_{ij}, \quad \langle H_i, E_j \rangle = \langle H_i, F_j \rangle = 0, \\
	\langle E_i, E_j \rangle = \langle F_i, F_j \rangle =  0,  \quad \text{and} \quad \langle E_i, F_j \rangle = \inv{d_i} \delta_{ij},
\end{split}
\end{gather*}
for all $i, j$ \cite[Theorem~2.2]{kac_1985}. When $\lieg = \gln$ we take $\langle , \rangle$ to be the non-degenerate trace bilinear form of the natural representation.
	
The bilinear form $\langle , \rangle$ induces an isomorphism of vector spaces $\nu\colon \mathfrak{h} \to \mathfrak{h}^*$ under which $H_i$ corresponds to the \textit{coroot} $\alpha_i^\vee = \inv{d_i} \alpha_i$. The induced form on $\mathfrak{h}^*$ satisfies
\begin{equation}\label{inner prod on roots}
	\langle \alpha_i, \alpha_j \rangle = d_i a_{ij}.
\end{equation}
%Matches SAGE convention!!! Same as 1.1.2 of Kac, but he uses coroots in Cartan subalgebra and his bracket notation refers to dual pairing
Since $a_{ii} = 2$, we must have $d_i = \langle \alpha_i, \alpha_i \rangle / 2$. Thus we obtain a formula for the \textit{Cartan integers}:
\begin{equation}\label{cartan ints as inn prod}
	a_{ij} = \langle \alpha_i^\vee, \alpha_j \rangle 
	= { 
		2 \langle \alpha_i^\vee, \alpha_j \rangle 
		\over 
		\langle \alpha_i, \alpha_i \rangle
	  }.
\end{equation} 
Notice the bilinear form induced by $\nu$ is normalized so that 
$$\langle \alpha_i, \alpha_i \rangle = 2d_i.$$
When $\lieg$ is simple\longer{, the Cartan matrix $A$ has entries $a_{ij} \in \{-3, -2, -1, 0, 2\}$, so without loss of generality we may assume that $D$ has entries $d_i \in \{1, 2, 3\}$, which implies} $\langle \alpha_i, \alpha_i \rangle = 2$ for \textit{short} roots.

For concreteness and convenience, we record some relevant Cartan matrices: 
\begin{align}\label{cartan mats}
\begin{gathered}
	A_n = 
	\begin{bmatrix*}[r]
	2  & -1     &        &        & \\
	-1 & 2      & -1     &        & \\
	   & \ddots & \ddots & \ddots & \\
	   &        & -1     & 2      & -1 \\
	   &        &        & -1     & 2
	\end{bmatrix*}, 
	\\ \\
	B_n = 
	\begin{bmatrix*}[r]
	\begin{matrix}
	& & &&\\
	& A_{n-1} &&& \\
	& & &&
	\end{matrix} \rvline
	& 
	\begin{matrix*}[c]
	0 \\ \vdots \\ 0 \\ -1
	\end{matrix*} \\
	\cmidrule(lr){1-1}
	\begin{matrix*}[l]
	0 & \cdots & 0 & -2
	\end{matrix*}
	& 2
	\end{bmatrix*}, 
	\quad \text{and} \quad 
	D_n = 
	\begin{bmatrix*}[r]
	\begin{matrix}
	& & &&&\\
	& A_{n-1} &&&& \\
	& & &&&
	\end{matrix} \rvline
	& 
	\begin{matrix*}[c]
	0 \\ \vdots \\ 0 \\ -1 \\ 0
	\end{matrix*} \\
	\cmidrule(lr){1-1}
	\begin{matrix*}[l]
	0 & \cdots & 0 & -1 & 0
	\end{matrix*}
	& 2
	\end{bmatrix*}.
\end{gathered}
\end{align}
We label the matrices by the Lie type of the root system to which they are associated. The corresponding diagonal   root lengths matrices are described by $d = (1, \ldots, 1)$ for the root systems of types $A_n, D_n$, and by $d = (2, \ldots, 2, 1)$ for type $B_n$.

\longer{If $\alpha \in \mathcal{Q}$, define the \textit{root space} 
$$\lieg_\alpha = \{ x \in \lieg \mid [h, x] = \alpha(h) x \text{ for all } h \in \mathfrak{h}\}.$$
The elements of $\Delta = \{ \alpha \in \mathcal{Q} \mid \alpha \neq 0, \lieg_\alpha \neq 0 \}$ are the \textit{roots} of $\lieg$. The intersection $\Delta^+ = \Delta \cap \mathcal{Q}^+$ denotes the set of \textit{positive roots}. The \textit{negative roots} are given by $\Delta^- = - \Delta^+$ and $\Delta = \Delta^+ \coprod \Delta^-$ \cite[Chapter 1]{kac_1985}. Distinct root spaces are orthogonal with respect to the bilinear form $\langle , \rangle$:
$$\langle \lieg_\alpha, \lieg_\beta \rangle \text{ if } \alpha \neq \beta \text{ and }  \langle \lieg_\alpha, \mathfrak{h} \rangle \text{ if } \alpha \neq 0$$
\cite[Theorem 2.2(c)]{kac_1985}. The Lie algebra $\lieg$ has a triangular decomposition with respect to its roots. As vector spaces, 
\begin{equation*}\label{triangular decomp g}
	\lieg = \big(\bigoplus_{\alpha < 0} \lieg_\alpha \big) \oplus \mathfrak{h} \oplus \big(\bigoplus_{\alpha > 0} \lieg_\alpha \big).
\end{equation*}}

We denote the half sum of the positive roots in $\mathfrak{h}^*$ by $\rho$. The \textit{Weyl vector} $\rho$ is uniquely characterized by $\langle \alpha_i^\vee, \rho \rangle = 1$. \longer{Thus its image $\rho^* \in \mathfrak{h}$ under $\inv{\nu}$ satisfies $\alpha_i(\rho^*) = d_i$. Concretely, if $b_i = \sum_j (\inv{A})_{ji} d_j$, then
\begin{equation}\label{weyl vector}
	\rho = \sum_{i} b_i \alpha_i^\vee \quad \text{and} \quad \rho^* = \sum_{i} b_i H_i.
\end{equation}

The \textit{fundamental weights} $\omega_i \in \mathfrak{h}^*$  are defined by $\omega_i(H_j) = \delta_{ij}$, or equivalently, $\langle \omega_i, \alpha_j^\vee \rangle = \delta_{ij}$. The $\omega_i$ form a basis of $\mathcal{P}$ and clearly
$$\alpha_i = \sum_j a_{ji} \omega_j.$$ 
Since $C = DA$ is symmetric $\alpha_i = \sum_j c_{ij} (\inv{d_j} \omega_j)$ and therefore
$$\omega_i = \sum_j (D\inv{A})_{ij} \alpha_j^\vee$$
because $C$ is invertible. Then
$\langle \omega_i, \omega_j \rangle = d_i (\inv{A})_{ij}$ follows from the definition of $\omega_i$. 

Now consider any weights $\lambda = \sum_i \lambda_i \omega_i$ and $\mu = \sum_i \mu_i \omega_i$, and notice  $\lambda(H_i) = \lambda_i$ and similarly $\mu(H_i) = \mu_i$. Therefore
\begin{equation}\label{scalar product of weights}
	\langle \lambda, \mu \rangle = \sum_{ij} \lambda_i \mu_j \langle \omega_i, \omega_j \rangle = \sum_{ij} (D\inv{A})_{ij} \lambda(H_i) \mu(H_j).
\end{equation}}

\paragraph{Casimir element}

Let $X_\alpha$ denote any basis of $\lieg$, and let $X^\alpha$ denote the corresponding dual basis with respect to $\langle \cdot, \cdot \rangle$. The next formula uniquely characterizes the \textit{Casimir element}
\begin{equation}\label{casimir elt}
C = \sum_{\alpha} X_{\alpha}  X^{\alpha}  = \sum_{\alpha} X^{\alpha}  X_{\alpha} \in \Ug.
\end{equation}
The Casimir element is in fact canonical and central \cite[Theorem~10.2]{Bump}. In addition, $C$ acts as the scalar 
\begin{equation}\label{casimir eigenvalues}
	\chi_{\lambda}(C) = \langle \lambda, \lambda + 2\rho\rangle
\end{equation}
on any irreducible $\Ug$-module with highest weight $\lambda$ \cite[Corollary~2.6]{kac_1985}. 


\paragraph{Quantum groups and their representations} 

Throughout this work, the term ``quantum group'' refers to an associative Hopf algebra $\Uqg$ as presented in \cite[Definition~9.1.1]{chari_pressley_1994}. \longer{For convenience, we reproduce the definition below. 

Let $\lieg$ denote a semisimple Lie algebra and let $A$ denote its generalized Cartan matrix with the diagonal matrix $D = \mathrm{diag}(d_1, \ldots, d_r)$ such that $DA$ is symmetric. Let $q$ be \textit{indeterminate} and write $q_i = q^{d_i}$.
	The \textit{quantum group} $\Uqg$ is the associative unital algebra over $\mathbb{C}(q)$ generated by the elements $E_i, F_i, K_i$, and $\inv{K_i}$, for $i = 1, \ldots, r$, subject to the relations:
\begin{equation}\label{uq rels}
\begin{gathered}
K_i K_j = K_j K_i, \quad K_i \inv{K_i} = \inv{K_i} K_i = 1, \\
K_i E_j \inv{K_i} = q_i^{a_{ij}} E_j, \quad K_i 
F_j \inv{K_i} = q_i^{-a_{ij}} F_j,  \\
E_i F_j - F_j E_i = \delta_{ij} \frac{K_i - \inv{K_i}}{q_i - \inv{q_i}},
\end{gathered}	
\end{equation}
together with the $q$-Serre relations for $i \neq j$,
\begin{equation}\label{uq Serre rels}
	\sum_{k = 0}^{1-a_{ij}} (-1)^k 
	\begin{bmatrix}
	1 - a_{ij} \\ k
	\end{bmatrix}_{q_i} 
	X_i^k X_j X_i^{1-a_{ij}-k} = 0.
\end{equation}
In the last equality every $X$ is either an $E$ or an $F$. The $q$-integer is given by $[n]_{q_i} = \frac{q_i^n - q_i^{-n}}{q_i - \inv{q_i}}$, the $q$-factorial $[n]_{q_i}! = [n]_{q_i}\cdots [1]_{q_i}$, and the $q$-binomial coefficient is defined analogously.} We note the following identity is often useful for verifying $q$-Serre relations when $a_{ij} = -1$. Writing $[A, B]_q = AB - qBA$, we have
\begin{align}\label{alt uq Serre rels}
\begin{split}
	\sum_{k = 0}^{1-a_{ij}} (-1)^k 
	\begin{bmatrix}
	1 - a_{ij} \\ k
	\end{bmatrix}_{q_i} 
	X_i^k X_j X_i^{1-a_{ij}-k} 
		&= X_i (X_i X_j - q_i X_j X_i) - \inv{q_i} (X_i X_j - q_i X_j X_i) X_i \\
		&= [X_i, [X_i, X_j]_{q_i}]_{\inv{q_i}}.
\end{split}
\end{align}

Unless otherwise stated, we assume that $\Uqg$ is equipped with the co-algebra structure defined by the comultiplication map $\Delta\colon \Uqg \to \Uqg^{\otimes 2}$ satisfying
\begin{align}\label{delta convention}
	\begin{split}
		\Delta(E_i) &= E_i \otimes K_i + 1 \otimes E_i \\
		\Delta(F_i) &= F_i \otimes 1 + \kinv \otimes F_i, 
		\quad \text{and} \\
		\Delta(K_i) &= K_i \otimes K_i,
	\end{split}
\end{align}
as in \cite{lzz_2010}. The choice of comultiplication convention is important in \ddichotomy{\Cref{type A duality ch,orthogonal duality ch}}{defining commuting module actions}, where different conventions are needed in order to ensure that relevant quantum groups induce commuting endomorphism subalgebras.

In this work, we only consider finite-dimensional type $(1, \ldots, 1)$ modules for the quantum groups $\Uqg$. Refer to Chapters~9 and~10 in \cite{chari_pressley_1994} for definitions. Every type $(1, \ldots, 1)$ finite-dimensional $\Uqg$-module is semisimple \cite[Theorem~5.17]{J} and each simple $\Uqg$-module is in one-to-one correspondence with a $\lieg$-module parametrized by a dominant weight of $\lieg$ \cite[Theorem~5.10]{J}. Moreover,  corresponding modules have the same weight multiplicities \cite[Lemma~5.14]{J}.
%\end{document}
